On the Problem of Computing the Probability of Regular Sets of Trees

We consider the problem of computing the probability of regular languages of infinite trees with respect to the natural coin-flipping measure. We propose an algorithm which computes the probability of languages recognizable by \emph{game automata}. In particular this algorithm is applicable to all deterministic automata. We then use the algorithm to prove through examples three properties of measure: (1) there exist regular sets having irrational probability, (2) there exist comeager regular sets having probability $0$ and (3) the probability of \emph{game languages} $W_{i,k}$, from automata theory, is $0$ if $k$ is odd and is $1$ otherwise.

==> app_tech.tex <==
For the sake of consistency we include a brief exposition of monadic second order logic (MSO). A standard reference is \cite{thomas96}. 
%The set $\{L,R\}^*$ of finite words  over the alphabet $\{L,R\}$ is called the \emph{full binary tree} and each $w\!\in\!\{L,R\}^*$ is referred to as a \emph{vertex}.
The functions $\SuccL$  ($w\mapsto w.L$) and $\SuccR$ ($w\mapsto w.R$) are called \emph{successor operations}. %Given a finite alphabet $\Sigma$ the function space $(\{L,R\}^*\rightarrow \Sigma)$ is denoted by $\trees{\Sigma}$ and an element $t\!\in\!\trees{\Sigma}$ is called a $\Sigma$-labeled tree, or just a $\Sigma$-tree. 
%We identify $\{0,1\}$-labeled trees, seen as characteristic functions, with sets of vertices. A tree $t\!\in\!\trees{\Sigma}$ is called \emph{regular} if it has only finitely many subtrees up-to isomorphism. The space $\trees{\Sigma}$ has a natural topology homeomorphic to the Cantor space. A basis for the topology consists of clopen sets of $\Sigma$-trees extending a given finite prefix.  
The language of MSO 
%is given by the following grammar
%$$\phi::= x\mid X \mid x\!\in\! X \mid \SuccL(x) \mid \SuccR(x) \mid \neg\phi \mid \phi\vee \phi \mid \forall x.\phi \mid \forall X.\phi$$
%consisting
consists of  \emph{first order variables} $x,y$ (ranging over vertices $w\!\in\!\{L,R\}^*$), second order variables $X,Y$ (ranging over sets of vertices $t\!\in\! \trees{0,1}$),  the set-theoretic membership relation $x\!\in\! X$, the operations  $\SuccL$ and $\SuccR$, the usual Boolean connectives ($\vee$, $\wedge$, $\neg)$, first order quantifiers ($\forall x.\phi$, $\exists x.\phi$) and  the second order quantifiers ($\forall X.\phi$, $\exists X.\phi$). In this paper we consider MSO formulas whose free variables are all second order. This is not a significant restriction since it is well known (see, e.g.,   \cite{thomas96}) how to present MSO as a purely second order (i.e., without first order variables and quantifiers) theory.  For a vector $\vv{Y}\!=\!(Y_1,\ldots,Y_n)$ and a variable $X$ we write $\phi(X,\vv{Y})$ to denote that $\phi$ has precisely $n+1$ free variables $X,Y_1,\dots, Y_n$. The set theoretic semantics of $\phi(X,\vv{Y})$ is the collection of $n+1$-tuples of $\{0,1\}$-trees $\langle t_0,t_1,\dots, t_n\rangle$ satisfying the formula $\phi$. Equivalently, $\phi(X,\vv{Y})$ defines a collection of $\Sigma$-trees with $\Sigma\!=\!\{0,1\}^{n+1}$. A subset $A\!\subseteq\! \trees{\Sigma}$ is \emph{regular} if it is definable by a MSO formula. Given a formula $\phi(X,\vv{Y})$ and a tuple $\vv{t}\!=\! \langle t_1,\dots, t_n\rangle$ of $\{0,1\}$-trees, the formula $\phi(X,\vv{t})$ with \emph{parameters} $\vv{t}$ denotes the \emph{section} $\{ t_0 \mid \langle t_0,t_1,\dots, t_n\rangle\! \in\! \phi(X,\vv{Y})\}\!\subseteq\! \trees{0,1}$. See Subsection \ref{related_work_intro} for an example how this semantics can be extended\footnote{Multiple nested applications of quantifiers  $\forall^{=1}X.\phi$ and  $\forall X.\phi$ potentially brings an issue of measurability of involved sets. This is not relevant for this paper, because we only the quantifier  $\forall^{=1}X.\phi$ only once. In general, this issue is not resolved by the methods of \cite{GMMS2014}, however measurability of involved sets follows from sufficiently strong set theoretical assumptions such as Projective Determinacy; however, we believe that the issue will find a more natural solution once we establish more facts about the decidability of fragments of the logic MSO+$\forall^{=1}X.\phi$.} to the instance of the quantifier  $\forall^{=1}X.\phi$.%Note that $\phi(X,\vv{t})$ needs not be regular, but is regular when $\vv{t}$ is a regular tree.


==> failvv_app3.tex <==
\subsection{Computations for the language $L_2$.} The language $L_2$ was defined in Section \ref{fail_vv} (see also Figure \ref{gvv_2}). We also computed there the probability of $L_2$ using elementary ad hoc considerations. Here we will compute again the probability of $L_2$ using Algorithm \ref{alg2} and the tool {\tt qepcad} \cite{tool:qepcad}. %we will show that that the language $L_2$ satisfies requirements of Example \ref{prop_example_1}, that is the measure of $L_2$ is not rational. 
%An ad hoc argument showing irrationality of the measure of $L_2$ was already presented in Section \ref{fail_vv}. 
As shown in Section \ref{fail_vv}, the measure of language $L_2$ is described by the following system of fixed--point equations
\[\left\{
\begin{array}{lcl} 
x_1 &  \stackrel{\mu}{=} & \frac{1}{3} + \frac{2}{3}x_1^2\\
x_2 &  \stackrel{\mu}{=} & \frac{1}{3}x_1^2 + \frac{2}{3}x_2^2
\end{array}
\right.
\]
\noindent
This translates to the following {\tt qepcad} code:
%This relatively simple system of equations can be analyzed by ad hoc methods, see Subsection \ref{subsection:irrational}. Nevertheless, we will analyze this system in the tool {\tt qepcad} (\cite{tool:qepcad}) using a simple computational scheme, which was applied in Subsection \ref{subsection:linfty}.
\begin{lstlisting}
(A x1prime) 
[
    [x1 = 1/3 + 2/3 x1^2] /\ 
    [x1prime = 1/3 + 2/3 x1prime^2 ==> x1prime >= x1 ]
].
\end{lstlisting}

\vspace{-26pt}
The above formula $\phi_1(x_1)$, written in a formalized language of {\tt qepcad}, expresses that $x_1$ is the smallest solution to the first equation. The solution generated by the tool is $2x_1 - 1 = 0$.
Using this information we get the next formula $\phi_2(x_2)$, saying that $x_2$ is the least solution of the system of fixed point equations satisfying the inequality $x_2\leq 1$.  
\begin{lstlisting}
(E x1)(A x2prime)(A x1prime)
[   
    [2 x1 - 1 = 0] /\ 
    [x2 = 1/3 x1^2 + 2/3 x2^2] /\
    [x2 <= 1] /\
    [
        [
            [2 x1prime - 1 = 0] /\ 
            [x2prime = 1/3 x1prime^2 + 2/3 x2prime^2] /\
            [x2prime <= 1] 
        ] ==> 
        [x2prime >= x2]
     ]
].
\end{lstlisting}

\vspace{-26pt}
\noindent
The tool {\tt qepcad} reduces the above formula $\phi_2(x_2)$ to a quantifier free expression
\begin{lstlisting}
x2 - 1 < 0 /\ 8 x2^2 - 12 x2 + 1 = 0
\end{lstlisting}

\vspace{-22pt}
\noindent
which in turn can be easily solved analytically. The formula is satisfied by exactly one 
$x = \frac{1}{4}(3-\sqrt{7})$, which is irrational and amounts approximately to $0.088$.



\subsection{Computations for the language $L_3$} 
\label{l3}
The language $L_3$ was defined in the first  paragraph of Section \ref{fail_vv}. 
This language is the third upper approximation of the language $L_\infty$ defined in the same section. One can visualize the new state and transition as shown in Figure \ref{gvv_4}.
%is described in the following figure
\input{pictures/gvv_picture4}

According to Theorem \ref{bellman}, the measure of language $L_3$ is equal to the value of the MBP ${\mathcal M}_3$, which 
is still simple enough, so that it can be analyzed directly by ad hoc methods. The MBP $\mathcal{M}_3$ corresponding to $\mathcal{A}_3$ extends the MBP $\mathcal{M}_2$ of the previous example with the probabilistic state $s_{q_3}$ and the three $\forall$-branching states $s_{q_3,a}$, $s_{q_3,b}$ and $s_{q_3,c}$. The new part of the automaton $\mathcal{A}_3$ is depicted in Figure \ref{gvv_2} (left). Noting the four new states are not reachable by the other eight states already present in $\mathcal{M}_2$, we already know that $val_{q_2}\!=\!\frac{1}{4}(3-\sqrt{7})$. Hence we can consider the simplified system of fixed-point equations $\mu \vec{x}.g(\vec{x})$ for calculating the values $val\!=\!(val_{q_3}, val_{q_{3},a}, val_{q_{3},b}, val_{{q_3},c})$ where $g$ is defined in Figure \ref{gvv_2} (right).
Hence the value $val_{q_3}$ is the least solution in $[0,1]$ of the equation 
\[ x = \frac{1}{3}(\frac{1}{4}(3-\sqrt{7}))^2 + \frac{2}{3}x^2, \]
which is equal to $\frac{1}{4}(3-\sqrt{1+3\sqrt{7}})$.

We will obtain the above conclusion using our computational scheme and the tool {\tt qepcad}. For this sake we will analyze the MBP ${\mathcal M}_3$ from scratch, first translating it into 
a system of 12 fixed-point equations. 
\begin{center}
$val = \begin{pmatrix} 
val_{s_{q_1}}\\
val_{s_{q_1,a}}\\
val_{s_{q_1,b}}\\
val_{s_{q_1,c}}\\
val_{s_{q_2}}\\
val_{s_{q_2,a}}\\
val_{s_{q_2,b}}\\
val_{s_{q_2,c}}\\
val_{s_{q_3}}\\
val_{s_{q_3,a}}\\
val_{s_{q_3,b}}\\
val_{s_{q_3,c}}\\
\end{pmatrix} \ \   \textnormal{ and } \ \ 
g(\begin{pmatrix} 
y_1\\
y_2\\
y_3\\
y_4\\
y_5 \\
y_6 \\
y_7 \\
y_8 \\
y_9 \\
y_{10} \\
y_{11} \\
y_{12} 
\end{pmatrix}
) = 
\begin{pmatrix} 
\frac{1}{3} y_2 +  \frac{1}{3} y_3 + \frac{1}{3} y_4  \\
1 \cdot 1 \\
y_1 \cdot y_1 \\
y_1 \cdot y_1 \\
\frac{1}{3} y_6 +  \frac{1}{3} y_7 + \frac{1}{3} y_8  \\
y_1 \cdot y_1 \\
y_5 \cdot y_5 \\
y_5 \cdot y_5 \\
\frac{1}{3} y_{10} +  \frac{1}{3} y_{11} + \frac{1}{3}  y_{12}  \\
y_5 \cdot y_5 \\
y_9 \cdot y_9 \\
y_9 \cdot y_9 \\
\end{pmatrix}
$
\end{center}
After elementary reductions and reassigning of the variables $x_1\gets y_1, x_2\gets y_5, x_3\gets y_9$, the above equation is equivalent to the following system of equations
\[\left\{
\begin{array}{lcl} 
x_1 &  \stackrel{\mu}{=} & \frac{1}{3} + \frac{2}{3}x_1^2\\
x_2 &  \stackrel{\mu}{=} & \frac{1}{3}x_1^2 + \frac{2}{3}x_2^2\\
x_3 &  \stackrel{\mu}{=} & \frac{1}{3}x_2^2 + \frac{2}{3}x_3^2
\end{array}
\right.
\]

Like in the case of language $L_2$, we start the formal analysis in {\tt qepcad} from the case of $\phi_1(x_1)$ characterizing the least solution to the first equation. 
\begin{lstlisting}
(A x1prime) 
[
    [x1 = 1/3 + 2/3 x1^2] /\ 
    [x1prime = 1/3 + 2/3 x1prime^2 ==> x1prime >= x1 ]
].
\end{lstlisting}
\vspace{-25pt}
The solver {\tt qepcad} gives us solution $2x_1 - 1 = 0$, which we use to write down the formula $\phi_2(x_2)$, describing  $x_2$ as the least solution to the second equation. 
\begin{lstlisting}
(E x1)(A x2prime)(A x1prime)
[   
    [2 x1 - 1 = 0] /\ 
    [x2 = 1/3 x1^2 + 2/3 x2^2] /\
    [x2 <= 1] /\
    [
        [
            [2 x1prime - 1 = 0] /\ 
            [x2prime <= 1] /\
            [x2prime = 1/3 x1prime^2 + 2/3 x2prime^2]
        ] ==> 
        [x2prime >= x2]
     ]
].
\end{lstlisting}
\vspace{-25pt}
As we already computed before, the formula $\phi_2(x_2)$ translates to a quantifier free expression
\begin{lstlisting}
x2 - 1 < 0 /\ 8 x2^2 - 12 x2 + 1 = 0
\end{lstlisting}
\vspace{-25pt}
Below in formula $\phi_3(x_3)$ we characterize $x_3$ as the least solution to the third equation. In the formula we use the above quantifier--free translation of the formula $\phi_2(x_2)$.  
This leads to the following formulation of $\phi_3(x_3)$.  
\begin{lstlisting}
(E x2)(A x3prime)(A x2prime)
[   
    [x2 - 1 < 0 /\ 8 x2^2 - 12 x2 + 1 = 0] /\ 
    [x3 = 1/3 x2^2 + 2/3 x3^2] /\
    [x3 <= 1] /\
    [
        [
            [x2prime - 1 < 0 /\ 8 x2prime^2 - 12 x2prime + 1 = 0] /\ 
            [x3prime <= 1] /\
            [x3prime = 1/3 x2prime^2 + 2/3 x3prime^2]
        ] ==> 
        [x3prime >= x3]
     ]
].
\end{lstlisting}
The formula $\phi_3(x_3)$ is translated by {\tt qepcad} to the following quantifier free expression
\begin{lstlisting}
x3 - 1 < 0 /\ 256 x3^4 - 768 x3^3 + 832 x3^2 - 384 x3 + 1 = 0
\end{lstlisting}

\vspace{-25pt}
\noindent
The only real solution is $x_3=\frac{1}{4}(3-\sqrt{1+3\sqrt{7}})$, which is approximately $0.0026$. This example shows in particular, that $x_3$ is not a quadratic irrational. In the case of the language $L_2$, the measure was expressible just with square roots of rational numbers. %\todo{I have no real reason to think so, but somehow find the speed of convergence as a potentially interesting topic. Here we have 1 decimal figure per iteration (so far).}


\begin{comment}
\subsection{Computations for the language $L_\infty$.}
The language $L_\infty$ was defined in Section \ref{failvv}. %the following two states
%\input{pictures/gvv_picture3} 
The measure of language $L_\infty$ is described by the following system of equations, which was introduced in Section \ref{failvv}.
\[\left\{
\begin{array}{lcl} 
x_1 &  \stackrel{\mu}{=}  & \frac{1}{3}x_2^2 + \frac{2}{3}x_1^2\\
x_2 &  \stackrel{\mu}{=}  & \frac{1}{3}x_2^2 + \frac{2}{3}x_1^2
\end{array}
\right.
\]
As in the above examples we start from a formula $\psi_1(x_1,x_2)$ characterizing $x_1$ as the least solution to the first equation. In the previous examples regarding measures of languages $L_2$ and $L_3$, the variable $x_2$ was not present in the formula $\phi_1$. Here it plays a role of a parameter. 
\begin{lstlisting}
(A x1prime) 
[
    [x1 = 1/3 x2^2 + 2/3 x1^2] /\ 
    [x1prime = 1/3 x2^2 + 2/3 x1prime^2 ==> x1prime >= x1 ]
].
\end{lstlisting}
The solver {\tt qepcad} translates $\psi_1(x_1,x_2)$ into the following quantifier free formula
\begin{lstlisting}
4 x1 - 3 <= 0 /\ x2^2 + 2 x1^2 - 3 x1 = 0
\end{lstlisting}
We use this translation in order to write down a formula $\psi_2(x_2)$ characterizing $x_2$ as the greatest solution to the second equation.  
\begin{lstlisting}
(E x1)(A x2prime)(A x1prime)
[   
    [4 x1 - 3 <= 0 /\ x2^2 + 2 x1^2 - 3 x1 = 0] /\
    [x2 = 1/3 x2^2 + 2/3 x1^2] /\
    [
        [
            [4 x1prime - 3 <= 0 /\ x2prime^2 + 2 x1prime^2 - 3 x1prime = 0] /\ 
            [x2prime = 1/3 x2prime^2 + 2/3 x1prime^2]
        ] ==> 
        [x2prime <= x2]
     ]
].
\end{lstlisting}
The solver {\tt qepcad} translates $\psi_2(x_2)$ to the following quantifier free expression
\begin{lstlisting}
x_2 = 0
\end{lstlisting}
This means that the measure of the language $L_\infty$ is $0$.  We also verify a Proposition formulated in Section \ref{failvv}.

\begin{repproposition}{propmeag}
\propmeag
\end{repproposition}
\begin{proof}
The proof consists of unfolding of the definition of a comeager set. From the definition it is enough to verify that the complement of $L$ is meager. Notice, that $t\not\in L$ if and only if $t\not\in L_n$ for certain $n\in\omega$. Hence, it is enough to prove that for every $n\in\omega$ the set $\Tr_{\{a,b,c\}}\setminus L_n$ is nowhere dense. That is, we have to show that for every non--empty open set $U\subset\Tr_{\{a,b,c\}}\setminus L_n$ there exists $V\subset U$, an open subset, such that $V\subset L_n$. We can assume that $U$ is a set of trees extending certain prefix $p$ of the binary tree. As $V$ we take a set of trees which extends a prefix $q$, where $q$ is an extension of $p$ by $n$ frontiers consisting of letters $a$. 
\end{proof}
\end{comment}

\subsection{Language $L_\infty$ is comeager}
\label{linfty}
\begin{repproposition}{propmeag}
\propmeag
\end{repproposition}  
\begin{proof}
The proof consists of unfolding of the definition of a comeager set. From the definition it is enough to verify that the complement of $L$ is meager. Notice, that $t\not\in L$ if and only if $t\not\in L_n$ for certain $n\in\omega$. Hence, it is enough to prove that for every $n\in\omega$ the set $\Tr_{\{a,b,c\}}\setminus L_n$ is nowhere dense. That is, we have to show that for every non--empty open set $U\subset\Tr_{\{a,b,c\}}\setminus L_n$ there exists $V\subset U$, an open subset, such that $V\subset L_n$. We can assume that $U$ is a set of trees extending certain prefix $p$ of the binary tree. As $V$ we take a set of trees which extends a prefix $q$, where $q$ is an extension of $p$ by $n$ frontiers consisting of letters $a$. 
\end{proof}


==> wik_app.tex <==
%\newcommand{\wikdet}{For every $k\geq 3$ holds \[ \det(A_k) = (-1)^{k-1}\frac{1}{k}. \] } 
\begin{replemma}{lemma:wikdet}
\wikdet
\end{replemma}

\noindent
Before the proof let us consider a special of $k=3$ . Then $ A_{3} = 
\begin{pmatrix} 
-\frac{2}{3}  & \frac{1}{3} \\
\frac{1}{3} & -\frac{2}{3}
\end{pmatrix}$, hence $\det(A_3)=\frac{4}{9}-\frac{1}{9}=\frac{3}{9}=\frac{1}{3}$. Moreover, one can notice that if we do not limit attention to the case $x_k=0$, then the system of equations has infinitely many solutions, because the matrix $\begin{pmatrix} 
-\frac{2}{3}  & \frac{1}{3} & \frac{1}{3} \\
\frac{1}{3} & -\frac{2}{3} & \frac{1}{3} \\
\frac{1}{3} & \frac{1}{3} & -\frac{2}{3}
\end{pmatrix}$ has determinant equal to $0$.

%\label{comp_wik}
%In this part of the Appendix we prove
%\begin{replemma}{lemma:wikdet}
%\wikdet
%\end{replemma}

\begin{proof}(of Lemma \ref{lemma:wikdet})

We simplify the determinant of the $(k-1)\times (k-1)$ matrix $A_k$ in order to have $0$'s in the first row on all positions, with except of the first one. 
\[\det(A_k) = \det
\begin{pmatrix} 
-\frac{k-1}{k}  & \frac{1}{k}       &   \frac{1}{k} & \ldots & \frac{1}{k} \\
\frac{1}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{1}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[= \det
\begin{pmatrix} 
(-\frac{k-1}{k}-\frac{1}{k}) & (\frac{1}{k}+\frac{k-1}{k})   &  0 & \ldots & 0 \\
\frac{1}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{1}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[ = \det
\begin{pmatrix} 
-1  & 1       &   0 & \ldots & 0 \\
\frac{1}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{1}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[= \det
\begin{pmatrix} 
-1  & 1-1       &   0 & \ldots & 0 \\
\frac{1}{k}     & (-\frac{k-1}{k}+\frac{1}{k})    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{1}{k}     & (\frac{1}{k}+\frac{1}{k})       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[= \det
\begin{pmatrix} 
-1  & 0       &   0 & \ldots & 0 \\
\frac{1}{k}     & -\frac{k-2}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{1}{k}     & \frac{2}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix}.
\]

Having $0$'s in the first row we unfold the determinant with respect to this row. The next determinant 
is of the size $(k-2)\times (k-2)$. Again, we aim to have $0$'s in the first row on all positions, with except of the first one. 

\[(-1) \det
\begin{pmatrix} 
-\frac{k-2}{k} & \frac{1}{k}  &  \frac{1}{k} & \ldots & \frac{1}{k} \\
\frac{2}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{2}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[ = (-1) \det
\begin{pmatrix} 
-1  & 1       &   0 & \ldots & 0 \\
\frac{2}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{2}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[= (-1) \det
\begin{pmatrix} 
-1  & 1-1       &   0 & \ldots & 0 \\
\frac{2}{k}     & (-\frac{k-1}{k}+\frac{2}{k})    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{2}{k}     & (\frac{1}{k}+\frac{2}{k})       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[ = (-1) \det
\begin{pmatrix} 
-1  & 0       &   0 & \ldots & 0 \\
\frac{2}{k}     & -\frac{k-3}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{2}{k}     & \frac{3}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix}.
\]

Now we are ready to again unfold the determinant with respect to the first row. In the following computations we deal 
with the matrix of the size $(k-3)\times (k-3)$. 

\[(-1)^2 \det
\begin{pmatrix} 
-\frac{k-3}{k} & \frac{1}{k}  &  \frac{1}{k} & \ldots & \frac{1}{k} \\
\frac{3}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{3}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[ = (-1)^2 \det
\begin{pmatrix} 
-1  & 1       &   0 & \ldots & 0 \\
\frac{3}{k}     & -\frac{k-1}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{3}{k}     & \frac{1}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[= (-1)^2 \det
\begin{pmatrix} 
-1  & 1-1       &   0 & \ldots & 0 \\
\frac{3}{k}     & (-\frac{k-1}{k}+\frac{3}{k})    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{3}{k}     & (\frac{1}{k}+\frac{3}{k})       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} \]
\[= (-1)^2 \det
\begin{pmatrix} 
-1  & 0       &   0 & \ldots & 0 \\
\frac{3}{k}     & -\frac{k-4}{k}    &   \frac{1}{k} & \ldots & \frac{1}{k} \\
& \vdots & \\
\frac{3}{k}     & \frac{4}{k}       &   \frac{1}{k} & \ldots & -\frac{k-1}{k}
\end{pmatrix} = \cdots
\]

Finally, after $k-3$ steps, we are ending up with a determinant of the size $2\times 2$:

\[
(-1)^{k-3} \det
\begin{pmatrix} 
-1  & 1  \\
\frac{k-2}{k}     & -\frac{k-1}{k} 
\end{pmatrix} = (-1)^{k-3}(\frac{k-1}{k}-\frac{k-2}{k}) = (-1)^{k-3}\frac{1}{k}.
\]

\end{proof}


